A Challenger to GPT-4V? Early Explorations of Gemini in Visual Expertise

The surge of interest towards Multi-modal Large Language Models (MLLMs), e.g., GPT-4V(ision) from OpenAI, has marked a significant trend in both academia and industry. They endow Large Language Models (LLMs) with powerful capabilities in visual understanding, enabling them to tackle diverse multi-modal tasks. Very recently, Google released Gemini, its newest and most capable MLLM built from the ground up for multi-modality. In light of the superior reasoning capabilities, can Gemini challenge GPT-4V's leading position in multi-modal learning? In this paper, we present a preliminary exploration of Gemini Pro's visual understanding proficiency, which comprehensively covers four domains: fundamental perception, advanced cognition, challenging vision tasks, and various expert capacities. We compare Gemini Pro with the state-of-the-art GPT-4V to evaluate its upper limits, along with the latest open-sourced MLLM, Sphinx, which reveals the gap between manual efforts and black-box systems. The qualitative samples indicate that, while GPT-4V and Gemini showcase different answering styles and preferences, they can exhibit comparable visual reasoning capabilities, and Sphinx still trails behind them concerning domain generalizability. Specifically, GPT-4V tends to elaborate detailed explanations and intermediate steps, and Gemini prefers to output a direct and concise answer. The quantitative evaluation on the popular MME benchmark also demonstrates the potential of Gemini to be a strong challenger to GPT-4V. Our early investigation of Gemini also observes some common issues of MLLMs, indicating that there still remains a considerable distance towards artificial general intelligence. Our project for tracking the progress of MLLM is released at https://github.com/BradyFU/Awesome-Multimodal-Large-Language-Models.

==> emotion.tex <==
\section{Emotion}
\label{sec:05emotion}
    % \item \textbf{Emotion.} This dimension examines the model's ability to understand and generate emotional responses. It involves tasks that assess emotion recognition from visual and textual cues and the generation of content that elicits specific emotional reactions. 


In the realm of artificial intelligence, the Emotion dimension is pivotal for models to interact with humans in a more natural and empathetic manner. It enables these models to not only interpret human emotions but also to respond in a manner that is contextually and emotionally appropriate.

In Section \ref{sec:05subsec:emoanalysis}, we will explore the models' ability to understand the emotion in the image, involving the tasks of facial expression analysis and image emotion analysis. 
In Section \ref{sec:05subsec:emogen}, we will examine the models' ability to generate content with emotion via the task of Emotion conditioned output. 

\subsection{Emotion Analysis}\label{sec:05subsec:emoanalysis}
Emotion Analysis involves the interpretation and identification of emotional states from various inputs such as facial expressions and postures. 
% This sub-dimension tests the model's ability to accurately discern subtle emotional cues, a key aspect of empathetic and effective communication.

\textbf{Facial expression analysis. }

\textbf{Image emotion analysis. }



\subsection{Emotion Generation}\label{sec:05subsec:emogen}
Emotion Generation focuses on the model's capacity to create responses that elicit specific emotional reactions, thus enabling the model to engage in interactions that are not just intellectually appropriate but also emotionally congruent.

\textbf{Emotion conditioned output.}


==> knowledge.tex <==
\section{Knowledge}
\label{sec:03knowledge}
    % \item \textbf{Knowledge.} This dimension evaluates the model's accumulation and application of information across various domains. It includes Commonsense Knowledge, Scientific Knowledge, Cultural Customs, and World Memory. Commonsense Knowledge encompasses everyday tasks like food recognition. Scientific Knowledge probes the model's understanding across diverse academic disciplines. Cultural Customs tests the model’s awareness of different cultural practices through recognition of wedding photos and festival activities from various cultures. World Memory is concerned with the recognition of global entities such as celebrities, landmarks, logos, artworks, flora and fauna, and movie posters.


\textit{Knowledge}, in the context of multi-modal large models, refers to the breadth and depth of information that the model can access, understand, and apply across various domains. This dimension is crucial as it underpins the model's ability to interpret, reason, and make informed decisions, directly impacting its performance in \textit{Cognition} and \textit{Expert Capacity} dimensions. 
For instance, a model well-versed in scientific knowledge can better tackle complex reasoning problems in science and technology domains. 
In this section, we divide \textit{Knowledge} into four sub-dimensions based on the functional utility of information for multi-modal large models: commonsense, subject knowledge, multi-culture, and world memory. 
In this section, we explore the \textit{Knowledge} of MLLM on four sub-dimensions: commonsense, subject knowledge, multi-culture, and world memory. 

In Section \ref{sec03:subsec:commonsense}, we will examine the commonsense of Gemini and GPT4V, including the commonsense in physical laws and social norms.  
In Section \ref{sec03:subsec:subject}, we will assess the models' knowledge on some subjects, such as Mathematics, Physics, Chemistry and History. 
In Section \ref{sec03:subsec:multiculture}, we will explore the models' ability to understand multiculture.
In Section \ref{sec03:subsec:memory}, we delve into the models' fine-grained memory on the wolrd, such as landmark, logo, movie poster, celebrity and more. 

\subsection{Commonsense}\label{sec03:subsec:commonsense}
\textit{Commonsense} encompasses the everyday, practical knowledge that is generally assumed to be known by people. This includes basic concepts of the physical world, social norms, and simple heuristics that guide everyday decisions. For a multi-modal model, this dimension is essential for understanding and interacting in day-to-day scenarios, making the model relatable and effective in general applications.

\textbf{Physical laws.}

\textbf{Social norms.}



\subsection{Subject Knowledge}\label{sec03:subsec:subject}
\textit{Subject Knowledge} pertains to specialized information across various academic and professional fields. This includes disciplines like science, technology, mathematics, history, and more. 
In multi-modal models, this knowledge enables the handling of tasks that require specific domain expertise, thereby enhancing their applicability in specialized settings.

\textbf{Mathematics.}

\textbf{Physics.}

\textbf{Chemistry.}

\textbf{History.}


\subsection{Multiculture}\label{sec03:subsec:multiculture}
\textit{Multiculture} refers to the model's understanding of diverse cultural contexts, practices, and perspectives. This dimension is crucial in today’s globalized world, where cross-cultural interactions are common. A model with strong multi-cultural knowledge can navigate and interpret a myriad of cultural nuances, aiding in more inclusive and globally aware applications.

\textbf{Multicultural customs.}

\subsection{World Memory}\label{sec03:subsec:memory}
\textit{World Memory} involves the model's ability to recognize and recall global entities such as famous personalities, historical events, landmarks, and iconic images. This aspect of knowledge is essential for models to contextualize information within a global framework, making them relevant and informed participants in discussions about world affairs and history.

\textbf{Landmark.}

\textbf{Logo.}

\textbf{Movie Poster.}

\textbf{Celebrity.}

\textbf{Animal, plant and food.}
